Inference Time Style Control for Summarization

How to generate summaries of different styles without requiring corpora in the target styles, or training separate models? We present two novel methods that can be deployed during summary decoding on any pre-trained Transformer-based summarization model. (1) Decoder state adjustment instantly modifies decoder final states with externally trained style scorers, to iteratively refine the output against a target style. (2) Word unit prediction constrains the word usage to impose strong lexical control during generation. In experiments of summarizing with simplicity control, automatic evaluation and human judges both find our models producing outputs in simpler languages while still informative. We also generate news headlines with various ideological leanings, which can be distinguished by humans with a reasonable probability.

==> naacl2021_shuyang_style (camera-ready)/00_abstract.tex <==
%auto-ignore
\begin{abstract}

How to generate summaries of different styles without requiring corpora in the target styles, or training separate models? 
We present two novel methods that can be deployed during summary decoding on any pre-trained Transformer-based summarization model.
(1) \textit{Decoder state adjustment} instantly modifies decoder final states with externally trained style scorers, to iteratively refine the output against a target style. 
(2) \textit{Word unit prediction} constrains the word usage to impose strong lexical control during generation.
In experiments of summarizing with simplicity control,  automatic evaluation and human judges both find our models producing outputs in simpler languages while still informative. We also generate news headlines with various ideological leanings, which can be distinguished by humans with a reasonable probability.


\end{abstract}

==> naacl2021_shuyang_style (camera-ready)/01_introduction.tex <==
%auto-ignore
\section{Introduction}

Generating summaries with different language styles can benefit readers of varying literacy levels~\cite{chandrasekaran-etal-2020-overview} or interests~\cite{jin-etal-2020-hooks}. 
Significant progress has been made in abstractive summarization with large pre-trained Transformers~\cite{NIPS2019_9464,lewis-etal-2020-bart,zhang2019pegasus,raffel2019exploring,song19d}. 
However, style-controlled summarization is much less studied~\cite{chandrasekaran-etal-2020-overview},
and two key challenges have been identified:
(1) \textit{lack of parallel data}, 
and (2) \textit{expensive (re)training}, e.g., separate summarizers must be trained or fine-tuned for a pre-defined set of styles~\cite{zhang-etal-2018-shaped}.  
Both challenges call for inference time methods built upon trained summarization models, to adjust styles flexibly and efficiently.


\begin{figure}[t]
    \fontsize{9}{11}\selectfont
    \setlength{\tabcolsep}{0pt}
    \hspace{-1mm}
    \begin{tabular}{p{0.49\textwidth}}
        \toprule
        \textbf{Daily Mail Article}: $\ldots$ $\pmb{\big [}$ A 16-year-old \textcolor{gray}{who} was born a girl but identifies as a boy has been \textcolor{cyan!10!blue}{\textbf{granted the opportunity}} \textcolor{gray}{to go through male puberty thanks to} hormone treatment. $\pmb{\big ]}$
        $\ldots$ $\pmb{\big [}$ \textcolor{gray}{The transgender boy, who has felt as though he is living in the wrong body since he was a child,} has been given permission by a \textcolor{gray}{Brisbane-based} judge to receive testosterone injections $\pmb{\big ]}$ 
        $\ldots$ \\
        \midrule
        \textbf{(a) Decoder State Adjustment}:  $\pmb{\big [}$ Queensland teen has been granted hormone treatment. The 16-year-old was born a girl but identifies as a boy. $\pmb{\big ]}$
        $\ldots$
        $\pmb{\big [}$ A judge has granted the teen permission to receive testosterone injections. $\pmb{\big ]}$ $\ldots$ \\
        \textbf{(b) Word Unit Prediction}: A 16-year-old who was born a girl has been \textcolor{cyan!10!blue}{\textbf{given the right}} to go through male puberty. The transgender boy has lived in a female body since he was a $\ldots$ \\
        \bottomrule
    \end{tabular}
    \vspace{-1mm}
    \caption{ 
    Sample summaries generated by our style control methods via (a) adjusting decoder states with a simplicity scorer and (b) predicting simple words to use.
    \textcolor{gray}{\bf Gray} texts are produced by BART but removed after decoder state adjustment. Simplified words and their counterparts in the source are highlighted in \textcolor{cyan!10!blue}{\bf blue}. 
    }
    \label{fig:intro}
    \vspace{-2mm}
\end{figure}

To address these challenges, we investigate \textit{just-in-time style control techniques that can be directly applied to any pre-trained sequence-to-sequence (seq2seq) summarization model}. 
We study two methods that leverage external classifiers to favor the generation of words for a given style. 
First, \textbf{decoder state adjustment} is proposed to alter the decoder final states with feedback signaled by style scorers, which are trained to capture global property. 
Second, to offer stronger {\it lexical control}, we introduce \textbf{word unit prediction} that directly constrains the output vocabulary.
Example system outputs are displayed in Fig.~\ref{fig:intro}. 
Notably, our techniques are deployed at \textit{inference time} so that the summary style can be adaptively adjusted during decoding.


We experiment with two tasks: (1) {simplicity control for document summarization} with CNN/Daily Mail, and (2) {headline generation with various ideological stances} on news articles from the SemEval task~\cite{stein:2019i} and a newly curated corpus consisting of multi-perspective stories from AllSides\footnote{\url{www.allsides.com}}. 
In this work, the algorithms are experimented with the BART model~\cite{lewis-etal-2020-bart}, though they also work with other Transformer models. 
Both automatic and human evaluations show that our models produce summaries in simpler languages than competitive baselines, and the informativeness is on par with a vanilla BART. Moreover, headlines generated by our models embody stronger ideological leaning than nontrivial comparisons.\footnote{Our code and data are available at: \url{https://shuyangcao.github.io/projects/inference_style_control}.} 


==> naacl2021_shuyang_style (camera-ready)/02_related_work.tex <==
%auto-ignore
\section{Related Work}

\noindent \textbf{Summarizing documents into different styles} are mainly studied on news articles, where one appends style codes as extra embeddings to the encoder~\cite{fan-etal-2018-controllable}, or connects separate decoders with a shared encoder~\cite{zhang-etal-2018-shaped}. 
Similar to our work, \citet{jin-etal-2020-hooks} leverage large pre-trained seq2seq models, but they modify model architecture by adding extra style-specific parameters. 
Nonetheless, existing work requires training \textit{new} summarizers for different target styles or modifying the model structure. 
In contrast, our methods only affect decoder states or lexical choices during inference, allowing on-demand style adjustment for summary generation. 

\noindent \textbf{Style-controlled text generation} has received significant research attentions, especially where parallel data is scant~\cite{lample2018multipleattribute,shang-etal-2019-semi,He2020A}.
Typical solutions involve disentangling style representation from content representation, and are often built upon autoencoders~\cite{pmlr-v70-hu17e} with adversarial training objectives~\cite{NIPS2018_7959}. The target style is then plugged in during generation. 
Recently, \citet{Dathathri2020Plug} propose plug and play language models (\textsc{PPLM}s) to alter the generation style by modifying all key-value pairs in the Transformer, which requires heavy computation during inference. \citet{krause2020gedi} then employ a generative discriminator (GeDi) to improve efficiency. Our methods are more efficient since we only modify the decoder final states or curtail the vocabulary.


==> naacl2021_shuyang_style (camera-ready)/03_methods.tex <==
%auto-ignore
\section{Inference Time Style Control}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{figures/fig_stylecontrol.pdf}
    \vspace{-1mm}
    \caption{
    Just-in-time style control: 
    (1) Decoder state adjustment takes in a style score and iteratively updates $\mathbf{o}_{t}$; 
    (2) Word unit prediction controls the vocabulary. 
    }
    \label{fig:style_control}
    \vspace{-3mm}
\end{figure}


\subsection{Global Characteristic Control via Decoder State Adjustment} 
\label{subsec:global_control}


Given a style classifier $q(z \vert \cdot)$ that measures to which extent does the current generated summary resemble the style $z$, 
we use its estimate to adjust the final decoder layer's state $\mathbf{o}_t$ at step $t$ with gradient descent, as illustrated in Fig.~\ref{fig:style_control}. 
The output token is produced as $p(y_t \vert y_{1:t-1}, \mathbf{x}) = \text{softmax} ( \mathbf{W}_{e} \mathbf{o}_t )$, $\mathbf{W}_{e}$ is the embedding matrix. 

Concretely, to generate the $t$-th token, a style score of $q(z \vert \mathbf{y}_{1:t+2})$ is first computed. 
In addition to what have been generated up to step $t-1$, we also sample $y_t$ and two future tokens for style estimation. 
The decoder state is updated as follows:

\vspace{-1mm}
{
    \fontsize{10}{11}\selectfont
    \begin{equation}
        \mathbf{o}_t \gets \mathbf{o}_t - \lambda \nabla_{\mathbf{o}_t} \big[- q(z \vert \mathbf{y}_{1:t+2}) \big]
    \end{equation}
}%
%
where $\lambda$ is the step size. Gradient descent is run for $10$ iterations for document summarization and $30$ iterations for headline generation. 


Below, we define one discriminative and one generative style classifier, to illustrate the method.


\smallskip
\noindent \textbf{Discriminative Style Scorer.} 
We feed the tokens into a RoBERTa encoder~\cite{liu2019roberta} and use the contextualized representation of the \texttt{BOS} token, i.e., $\mathbf{h}_0$, to predict the style score as $p_{sty} (z \vert \cdot) = \mathrm{softmax} (\mathbf{W}_{s}\mathbf{h}_0)$, where $\mathbf{W}_{\ast}$ are learnable parameters in this paper. At step $t$ of summary decoding, the style score is estimated as:

\vspace{-1mm}
{
    \fontsize{10}{11}\selectfont
    \begin{equation}
        q(z \vert \mathbf{y}_{1:t+2}) = \log p_{sty}(z \vert \mathbf{y}_{1:t+2})
    \end{equation}
}%
For the discriminative style scorer, the step size $\lambda$ is set to $1.0$.

\smallskip
\noindent \textbf{Generative Language Model Scorer.}
We build a class-conditional language model (CC-LM) from texts prepended with special style-indicating tokens.
Concretely, the CC-LM yields probabilities $p_{LM} (y_{t^\prime} \vert \mathbf{y}_{1:t^\prime-1}, z)$ ($p_{LM}(y_{t^\prime}, z)$ for short), conditional on the previously generated tokens $\mathbf{y}_{1:t^\prime-1}$ and the style $z$.
As the summarizer's output probability $p(y_{t^\prime})$ should be close to the language model's estimate, the style score is defined as: 

\vspace{-5mm}
{
    \fontsize{10}{11}\selectfont
    \begin{equation}
        q(z \vert \mathbf{y}_{1:t+2}) = \frac{1}{t+2} \sum^{t+2}_{t^\prime=1} p_{LM}(y_{t^\prime}, z) \log p(y_{t^\prime})
    \end{equation}
}%
Here we use a step size $\lambda$ of $0.1$.


\subsection{Lexical Control via Word Unit Prediction} 
\label{subsec:lexical_control}

Lexical control is another tool for managing summary style, as word choice provides a strong signal of language style.
Given an input document, our goal is to predict a set of word units (e.g., the subwords used in BART pre-training) that can be used for summary generation. For instance, if the input contains ``affix'', we will predict ``stick'' to be used, while excluding the original word ``affix''. A similar idea has been used to expedite sequence generation~\cite{hashimoto-tsuruoka-2019-accelerated}, though our goal here is to calculate the possibilities of different lexical choices.

Concretely, after encoding the input $\mathbf{x}$ by RoBERTa, we take the average of all tokens' contextual representations, and pass it through a residual block~\cite{he2016deep} to get its final representation $\mathbf{\tilde{R}}$. We then compute a probability vector for all word units in the vocabulary as $\mathbf{p}^{r} = \text{sigmoid} (\mathbf{W}_r \mathbf{\tilde{R}})$. 
The top $v$ word units with the highest probabilities 
are selected and combined with entity names from the input to form the new vocabulary, from which the summary is generated.
We use $v=1000$ in all experiments. 


\smallskip
\noindent \textbf{Dynamic Prediction.} 
We also experiment with a dynamic version, where the word unit predictor further considers what have been generated up to a given step. In this way, the new vocabulary is updated every $m$ steps ($m=5$ for document summarization, and $m=3$ for headline generation).



==> naacl2021_shuyang_style (camera-ready)/04_doc_summ.tex <==
%auto-ignore
\section{Simplicity-controlled Document Summarization}

For experiments, we use BART fine-tuned on the CNN/DailyMail (CNN/DM)~\cite{NIPS2015_5945}, by following \citet{lewis-etal-2020-bart} for data preprocessing and splitting. The numbers of data in train, validation and test splits are $287{,}188$, $13{,}367$ and $11{,}490$, respectively.

We use paragraph pairs from normal and simple English Wikipedia articles in~\citet{hua-wang-2019-sentence} for {\it simplicity style scorer} and {\it class-conditional language model} training. We split the pairs into $86{,}467$, $10{,}778$, and $10{,}788$ for training, validation and testing, respectively. On the test set, our simplicity style scorer achieves an F1 score of $89.7$ and our class-conditional language model achieves a perplexity of $30.35$.

To learn the {\it word unit predictor}, for each paragraph pair, the predictor reads in the normal version and is trained to predict the word units used in the simple version.
For the {\it dynamic version}, it predicts which word units are used to generate the rest of the text, after every $5$ steps. Recalls for the two predictors on the test set are $81.5$ and $80.0$.%, respectively.

For comparison, we consider \textbf{\textsc{Reranking}} beams based on our style score at the last step. 
%
We also use a label-controlled (\textbf{\textsc{LblCtrl}}) baseline as described in \citet{niu-bansal-2018-polite}, where summaries in the training data are labeled as simple or normal by our scorer. 
%
We further compare with \textbf{\textsc{GeDi}} and two pipeline models: a style transfer model~\cite{pmlr-v70-hu17e} applied on the output of BART (\textbf{\textsc{CtrlGen}}) and a normal-to-simple translation model fine-tuned from BART (\textbf{\textsc{Trans}}), both trained on Wikipedia.
Finally, we consider \textbf{\textsc{LightLS}}~\cite{glavavs-vstajner:2015:ACL-IJCNLP}, a rule-based lexical simplification model.

\begin{table}[t]
\small
    \centering
    \setlength{\tabcolsep}{1.3pt}
    \begin{tabular}{lccccc}
    \toprule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Style}} & \textbf{Flu.} & \textbf{Cont.} \\
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-5}
        \cmidrule(lr){6-6}
        & \textbf{Simp.$\uparrow$} & \textbf{\%Simp.$\uparrow$} & \textbf{Rd.$\downarrow$} & \textbf{PPL$\downarrow$} & \textbf{BERT$\uparrow$} \\
        \midrule
        \textsc{BART} & 56.93 & 62.70 & 8.06 & 34.05 & 88.62 \\
        \midrule
        \textsc{Reranking} & 71.33 & 62.68 & 8.04 & 36.17 & 88.62 \\
        \textsc{LblCtrl} & 56.21 & 62.71 & 8.07 & 28.85 & 88.57 \\
        \textsc{CtrlGen} & 81.56 & 64.78 & 7.79 & 70.36 & 88.01 \\
        \textsc{Trans} & 59.78 & 63.03 & 7.99 & 33.17 & 88.46 \\
        \textsc{GeDi} & 71.33 & 62.57 & 7.88 & 33.48 & \textbf{88.79} \\
        \textsc{LightLS} & 69.02 & 64.92 & 7.72 & 76.37 & 86.98 \\
        \hdashline
        \multicolumn{6}{l}{\rule{0pt}{2ex}\bf Ours w/ Decoder State Adjustment}\\
        \textsc{Simp. Scorer} & 86.67 & 62.94 & 7.77 & 34.20 & 88.71 \\
        \textsc{Simp. CC-LM} & 75.04 & 64.27 & 7.69 & 30.49 & 88.73 \\
        \multicolumn{6}{l}{\bf Ours w/ Word Unit Prediction}\\
        \textsc{WordU} & \textbf{95.85} & 67.23 & \textbf{7.19} & \textbf{27.40} & 87.76 \\
        \textsc{Dynamic WordU} & 93.87 & \textbf{67.37} & 7.23 & 28.42 & 87.91 \\
        \bottomrule
    \end{tabular}
    \vspace{-1mm}
    \caption{
    Automatic evaluation on summarization with simplicity, with simplicity level by our scorer (Simp., probability multiplied by 100),  \% of words in the Dale-Chall simple word list (\%Simp.), Dale-Chall readability (Rd.), fluency by perplexity (PPL), and content metric by BERTScore (BERT). Our models are significantly better than the comparisons ($p < 0.005$) on simplicity and readability, except for \textsc{CtrlGen} and \textsc{LightLS}.
    }
    \label{tab:doc_summ_simplicity_auto_eval}
    \vspace{-2mm}
\end{table}


\smallskip
\noindent \textbf{Automatic Evaluation.}
Table~\ref{tab:doc_summ_simplicity_auto_eval} shows that \textit{our models' outputs have significantly better simplicity and readability while preserving fluency and a comparable amount of salient content}. 
Key metrics include simplicity level estimated by our scorer and Dale-Chall readability~\cite{chall1995readability}. 
We use GPT-2 perplexity~\cite{radford2019language} to measure fluency, and BERTScore~\cite{Zhang*2020BERTScore:} for content preservation. 
%
Our inference time style control modules can adaptively change the output style, and thus outperform reranking at the end of generation or using pipeline models. Moreover, by iteratively adjusting the decoder states, our methods deliver stronger style control than \textsc{GeDi}, which only adjusts the probability once per step.

When comparing among our models, we find that \textit{word unit prediction is more effective at lexical simplification than updating decoder states}, as demonstrated by the higher usage of simple words according to the Dale-Chall list. We believe that strong lexical control is achieved by directly pruning output vocabulary, whilst decoder state adjustment is more poised to capture global property, e.g., sentence compression as shown in Fig.~\ref{fig:intro}. Moreover, we compute the edit distance between our style-controlled system outputs and the summaries produced by the fine-tuned BART. We find that adjusting decoder states with style scorer and language model yields an edit distance of $45.7$ and $47.4$, compared to larger distances of $56.7$ and $54.3$ given by word unit prediction and with additional dynamic prediction. 



\smallskip
\noindent \textbf{Human Evaluation.}
We recruit three fluent English speakers to evaluate system summaries for \textbf{informativeness}---whether the summary covers important information from the input, and \textbf{fluency}---whether the summary is grammatical, 
on a scale of 1 (worst) to 5 (best). 
They then rank the summaries by \textbf{simplicity} level (ties are allowed). 
%
50 samples are randomly selected for evaluation, and system summaries are shuffled. 
As seen in Table~\ref{tab:simplicity_human_eval}, \textit{summaries by our models are considered simpler} than outputs of BART and \textsc{GeDi}, with better or comparable informativeness. 



\begin{table}[t]
    \small
    \centering
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{lcccc}
    \toprule
        \textbf{Model} & \textbf{Inf.$\uparrow$} & \textbf{Flu.$\uparrow$} & \textbf{Simp.R.$\downarrow$} & \textbf{Top 1$\uparrow$} \\
        \midrule
        \textsc{BART} & 4.45 & \textbf{4.90} & 2.19 & 19.0\% \\
        \textsc{GeDi} & 4.48 & 4.83 & 2.00 & 23.8\% \\
        \hdashline
        \rule{-2pt}{2ex}
        \textsc{Simp. Scorer} & \textbf{4.53} & 4.83 & 1.66{$^\ast$} & 48.4\% \\
        \textsc{Dynamic WordU}  & 4.36 & 4.84 & \textbf{1.65}{$^\ast$} & \textbf{57.9\%} \\
        \bottomrule
    \end{tabular}
    \vspace{-1mm}
    \caption{
    Human evaluation on informativeness (Inf.), fluency (Flu.), simplicity ranking (Simp.R.), and percentage of summaries ranked as simplest (Top 1). 
    Krippendorff's $\alpha$: 0.38, 0.22, and 0.16 (first three metrics). 
    $\ast$: significantly better than comparisons ($p < 0.005$). 
    }
    \label{tab:simplicity_human_eval}
    \vspace{-3mm}
\end{table}


==> naacl2021_shuyang_style (camera-ready)/05_head_gen.tex <==
%auto-ignore
\section{Ideology-controlled Headline Generation}

To generate news headlines of various ideological leanings, we use the \textbf{SemEval} Hyperpartisan News Detection dataset~\cite{stein:2019i}, where each article is labeled with a stance: \textit{left}, \textit{leaning left}, \textit{neutral}, \textit{leaning right}, or \textit{right}. Here, we combine left and leaning-left articles into one bucket, and similarly for right and leaning-right articles.
We use the lead paragraph as the input, and the headline as the target generation. The data is processed following~\citet{rush-etal-2015-neural}, and split into $346{,}985$ for training, $30{,}000$ each for validation and testing. Details of the ideology distribution for SemEval are in Appendix~\ref{append:semeval_allsides}.

We fine-tune BART and train ideology classifiers on the SemEval training set.
First, two binary {\it style scorers} are trained on headlines of left and right stances, with F1 scores of $76.1$ and $78.0$, respectively.
One {\it class-conditional language model} is trained on headlines with a stance token (left or right) prepended, achieving a perplexity of $54.7$.
To learn the {\it word unit predictor} for the left (and similarly for the right), we use samples that are labeled as left-leaning, treat the lead paragraph as the input, and then predict the word units used in the headline. Recalls for our predictors range from $77.8$ to $83.5$. 


\begin{table}[t]
\small
    \centering
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{lccccc}
    \toprule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Left}} & \multicolumn{2}{c}{\textbf{Right}} \\
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
        & \textbf{Ideol.} & \textbf{BERT} & \textbf{Ideol.} & \textbf{BERT}  \\
        \midrule
        \textsc{BART}  & 18.63 & 91.03 & 19.04 & 91.03 \\
        \midrule
        \textsc{Reranking} & 30.80 & 90.68 & 30.11 & 90.66 \\
        \textsc{LblCtrl} & 20.59 & \textbf{90.97} & 20.89 & \textbf{91.02} \\
        \textsc{GeDi} & 12.64 & 84.84 & 3.61 & 84.84 \\
        \hdashline
        \multicolumn{6}{l}{\rule{0pt}{2ex}\bf Ours w/ Decoder State Adjustment}\\
        \textsc{Ideol. Scorer} & \textbf{31.15} & 90.08 & \textbf{30.54} & 90.17 \\
        \textsc{Ideol. CC-LM} & 23.74 & 89.65 & 20.79 & 89.65 \\
        \multicolumn{6}{l}{\bf Ours w/ Word Unit Prediction}\\
        \textsc{WordU} & 21.30 & 89.64 & 20.42 & 90.13 \\
        \textsc{Dynamic WordU} & 21.53 & 89.49 & 20.09 & 90.19 \\
        \bottomrule
    \end{tabular}
    \vspace{-1mm}
    \caption{
    Ideological headline generation results.
    Using ideology scorer to update decoder states yields the highest ideology scores (multiplied by 100).  
    }
    \label{tab:ideology_auto_eval}
    \vspace{-1mm}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/fig_liwc.pdf}
    \vspace{-1mm}
    \caption{
    LIWC word usage changes of ``negate'' and ``affect'', compared to neutral headlines. In each subfigure, left and right panels correspond to left and right leaning stances. 
    }
    \label{fig:liwc}
    \vspace{-2mm}
\end{figure}

\smallskip
\noindent \textbf{Automatic Evaluation with SemEval.}
Table~\ref{tab:ideology_auto_eval} shows that \textit{our decoder state adjustment model with the ideology scorer obtains the highest ideology scores}, due to its effectiveness at capturing the global context---stance is often signaled by the joint selection of entities and sentiments. 

One might be interested in \textit{which words are favored for ideology-controlled generation}. To that end, we analyze the change of word usages with Linguistic Inquiry and Word Count (LIWC)~\cite{pennebaker2015development}. 
In Fig.~\ref{fig:liwc}, it can be seen that word unit prediction-based models generate more ``negations'', consistent with trends observed in human-written headlines. 
Meanwhile, models with decoder state adjustment and the baselines all use more ``affect'' words in both stances, indicating that they consider it easier to use explicit sentiments to demonstrate the stances.


\begin{table}[t]
    \small
    \setlength{\tabcolsep}{2pt}
    \centering
    \begin{tabular}{llllc}
    \toprule
        \textbf{Model} & \textbf{Rel.} & \textbf{Edit} & \textbf{Hmn} & \textbf{Hmn Acc.}\\
        \midrule
        Human & 4.01 & 12.24 & 60.8\% & 73.3\% \\
        \midrule
        \textsc{Reranking} & \textbf{4.71} & 3.90 & 24.5\% & 52.5\% \\
        \textsc{LblCtrl} & 4.70 & 2.30 & 11.6\% & \textbf{71.4\%} \\
        \hdashline
        \rule{-2pt}{2ex}
        \textsc{Ideol. Scorer} (ours) & 4.47 & \textbf{8.86}{$^\ast$} & \textbf{42.5\%}{$^\ast$} & 53.9\% \\
        \textsc{Dynamic WordU} (ours) & 4.66 & 4.20 & 25.8\% & 51.6\% \\
        \bottomrule
    \end{tabular}
    \vspace{-1mm}
    \caption{
    Human evaluation of ideology-controlled headline generation with relevance (Rel.), edit distance (Edit) between left and right headlines, \% of samples perceived as having different stances (Hmn), and (among them) accuracy of identified stances (Hmn Acc.). 
    Krippendorff's $\alpha$ of relevance: 0.48.
    $\ast$: significantly better than other models ($p < 0.005$).
    }
    \label{tab:ideology_human_eval}
    \vspace{-2mm}
\end{table}

\smallskip
\noindent \textbf{Human Evaluation with AllSides.} 
Given the low ideology scores in Table \ref{tab:ideology_auto_eval}, we further study \textit{if human can distinguish the stances in human-written and system generated headlines}. 
%
News clusters from \textbf{AllSides} are used, where each cluster focuses on one story, with multiple paragraph-headline pairs from publishers of \textit{left}, \textit{neutral}, and \textit{right} ideological leanings. We use the lead paragraph as the input, and collect $2{,}985$ clusters with samples written in all three stances. More details of the collection are in Appendix~\ref{append:semeval_allsides}.
%
We test and report results by using lead paragraphs from \textit{neural} articles as the input to construct headlines of \textit{left} and \textit{right} ideological stances. 
 
We randomly pick 80 samples and include, for each sample, two headlines of different stances generated by each system. 
%
Raters first score the \textbf{relevance} of the generated headlines to the neutral paragraph's headline, on a scale of $1$ to $5$. They then read each pair of headlines to decide whether they are written in different stances, and if so, to label them. 
%
Table~\ref{tab:ideology_human_eval} highlights the intrinsic difficulty of capturing ideological language usage: Even reference headlines are only distinguishable in $60.8\%$ of the cases, among which the stance identification accuracy is $73.3\%$.
%
In comparison, $42.5\%$ of the output pairs by the decoder state adjustment model can be distinguished, significantly higher than those of the baselines ($24.5\%$ and $11.6\%$). 
%
Sample outputs by our models are shown in Table~\ref{tab:sample_ideol}, with more outputs included in Appendix~\ref{append:sample_output}.

\begin{table}[t]
    \small
    \setlength{\tabcolsep}{0pt}
    \begin{tabular}{p{0.49\textwidth}}
    \toprule
    \textbf{Paragraph}: The Obama administration on Thursday rolled out new efforts aimed at curtailing gun violence $\ldots$ \\
    \midrule
        \textbf{\textsc{Reference}} \\
        \rowcolor{LeftBlue!60}
        $[$L$]$: obama offers new executive actions on gun control \\
        \rowcolor{red!15}
        $[$R$]$: administration announces new gun control measures, targets military surplus imports \\
        \midrule
        \textbf{\textsc{Ideol.Scorer}} \\
        \rowcolor{LeftBlue!60} $[$L$]$: u.s. moves to \textbf{curb gun violence} with new rules \\
        \rowcolor{red!15} $[$R$]$: obama admin to \textbf{tighten gun control laws} \\
        \midrule
        \textbf{\textsc{Dynamic WordU}} \\
        \rowcolor{LeftBlue!60} $[$L$]$: obama unveils new steps to \textbf{curb gun violence} \\
        \rowcolor{red!15} $[$R$]$: obama administration unveils new \textbf{gun control} measures \\
        \bottomrule
    \end{tabular}
    \vspace{-1mm}
    \caption{
    Sample generated headlines with left (shaded in \textcolor{LeftBlue!99}{\bf blue}) and right (\textcolor{red!60}{\bf red}) stances. Phrases that are typically used by a stance are in \textbf{bold}.
    }
    \label{tab:sample_ideol}
    \vspace{-2mm}
\end{table}


==> naacl2021_shuyang_style (camera-ready)/06_conclusion.tex <==
%auto-ignore
\section{Conclusion}

We present two just-in-time style control methods, which can be used in any Transformer-based summarization models. The decoder state adjustment technique modifies decoder final states based on externally trained style scorers. To gain stronger lexical control, word unit prediction directly narrows the vocabulary for generation. 
%
Human judges rate our system summaries to be simpler with better readability. We are also able to generate headlines with different ideological leanings.

==> naacl2021_shuyang_style (camera-ready)/07_acknowledgements.tex <==
%auto-ignore
\section*{Acknowledgements}
This research is supported in part by National Science Foundation through Grant IIS-1813341, and by the Office of the Director of National Intelligence (ODNI), Intelligence Advanced Research Projects Activity (IARPA), via contract \# FA8650-17-C-9116. The views and conclusions contained herein are those of the authors and should not be interpreted as necessarily representing the official policies, either expressed or implied, of ODNI, IARPA, or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for governmental purposes notwithstanding any copyright annotation therein. 
We thank all the anonymous reviewers for their constructive suggestions. 
